A Highly Efficient Distributed Deep Learning System For Automatic Speech Recognition

Modern Automatic Speech Recognition (ASR) systems rely on distributed deep learning to for quick training completion. To enable efficient distributed training, it is imperative that the training algorithms can converge with a large mini-batch size. In this work, we discovered that Asynchronous Decentralized Parallel Stochastic Gradient Descent (ADPSGD) can work with much larger batch size than commonly used Synchronous SGD (SSGD) algorithm. On commonly used public SWB-300 and SWB-2000 ASR datasets, ADPSGD can converge with a batch size 3X as large as the one used in SSGD, thus enable training at a much larger scale. Further, we proposed a Hierarchical-ADPSGD (H-ADPSGD) system in which learners on the same computing node construct a super learner via a fast allreduce implementation, and super learners deploy ADPSGD algorithm among themselves. On a 64 Nvidia V100 GPU cluster connected via a 100Gb/s Ethernet network, our system is able to train SWB-2000 to reach a 7.6% WER on the Hub5-2000 Switchboard (SWB) test-set and a 13.2% WER on the Call-home (CH) test-set in 5.2 hours. To the best of our knowledge, this is the fastest ASR training system that attains this level of model accuracy for SWB-2000 task to be ever reported in the literature.

==> Makefile <==
.SUFFIXES: .eps .pdf
LATEX=./colourlatex.sh pdflatex
BIBTEX=bibtex
FIG2DEV=fig2dev

MAIN=main
#SUP=supplementary
#BIBMAIN=acmsmall-sample-bibfile
BIBMAIN=mybib

all: $(MAIN).pdf #$(SUP).pdf #$(MAIN).ps

#FIGSEPS=$(shell ls -1 figs/*.eps)

#RESULTSEPS=$(shell ls -1 results/*.eps)

#EPS=$(FIGSEPS) $(RESULTSEPS)




MAINTEX=$(MAIN).tex \
    $(BIBMAIN).bib \

$(MAIN).pdf: $(MAINTEX) $(EPS) $(BIBMAIN).bbl
	@echo Compiling $(MAIN)
	@$(LATEX) $(MAIN)
	@$(MAKE) fixlabels

# SUPTEX=$(SUP).tex \
#     $(BIBMAIN).bib \

# $(SUP).pdf: $(SUPTEX) $(EPS) $(BIBMAIN).bbl
# 	@echo Compiling $(SUP)
# 	@$(LATEX) $(SUP)
# 	@$(MAKE) fixlabels
 

# $(MAIN).pdf: $(MAIN).dvi
# 	@dvipdfmx -p letter $(MAIN).dvi

# $(MAIN).ps: $(MAIN).dvi
# 	@dvips $(MAIN).dvi
# 	@pkill -HUP -f "^gv .*$@" || true


fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' $(MAIN).log),0)
	@echo $(MAIN) Compiling again to fix labels
	@$(LATEX) $(MAIN)
else
	@echo $(MAIN) Labels are correct
endif

$(BIBMAIN).bbl: $(BIBMAIN).bib
	@echo Compiling required EPS files
	#@make -C figs
	@echo Compiling main for bibliography
	@$(LATEX) $(MAIN)
	@echo Generating bibliography
	@$(BIBTEX) $(MAIN)
	@echo Recompiling main after generating bibliography
	@$(LATEX)  $(MAIN)
	@$(MAKE) fixlabels
	# @echo Compiling SUP for bibliography
	# @$(LATEX) $(SUP)
	# @echo Generating bibliography
	# @$(BIBTEX) $(SUP)
	# @echo Recompiling SUP after generating bibliography
	# @$(LATEX)  $(SUP)
	# @$(MAKE) fixlabels

%.eps.pdf: %.eps
	@echo "	" Converting $< to $(@)
	@epstopdf --outfile=figs/$(@) $<

clean:
	#@make -C figs clean
	@/bin/rm -f $(MAIN).ps $(MAIN).pdf *.aux *.dvi *.log *.bbl *.blg figs/*.pdf figures/plot/*.pdf *.toc *.out *.bak


==> Makefile_ <==
.SUFFIXES: .eps .pdf
LATEX=./colourlatex.sh pdflatex
BIBTEX=bibtex
FIG2DEV=fig2dev

MAIN=main
#SUP=supplementary
#BIBMAIN=acmsmall-sample-bibfile
BIBMAIN=refs

all: $(MAIN).pdf #$(SUP).pdf #$(MAIN).ps

#FIGSEPS=$(shell ls -1 figs/*.eps)

#RESULTSEPS=$(shell ls -1 results/*.eps)

#EPS=$(FIGSEPS) $(RESULTSEPS)




MAINTEX=$(MAIN).tex \
    $(BIBMAIN).bib \

$(MAIN).pdf: $(MAINTEX) $(EPS) $(BIBMAIN).bbl
	@echo Compiling $(MAIN)
	@$(LATEX) $(MAIN)
	@$(MAKE) fixlabels

# SUPTEX=$(SUP).tex \
#     $(BIBMAIN).bib \

# $(SUP).pdf: $(SUPTEX) $(EPS) $(BIBMAIN).bbl
# 	@echo Compiling $(SUP)
# 	@$(LATEX) $(SUP)
# 	@$(MAKE) fixlabels
 

# $(MAIN).pdf: $(MAIN).dvi
# 	@dvipdfmx -p letter $(MAIN).dvi

# $(MAIN).ps: $(MAIN).dvi
# 	@dvips $(MAIN).dvi
# 	@pkill -HUP -f "^gv .*$@" || true


fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' $(MAIN).log),0)
	@echo $(MAIN) Compiling again to fix labels
	@$(LATEX) $(MAIN)
else
	@echo $(MAIN) Labels are correct
endif

$(BIBMAIN).bbl: $(BIBMAIN).bib
	@echo Compiling required EPS files
	#@make -C figs
	@echo Compiling main for bibliography
	@$(LATEX) $(MAIN)
	@echo Generating bibliography
	@$(BIBTEX) $(MAIN)
	@echo Recompiling main after generating bibliography
	@$(LATEX)  $(MAIN)
	@$(MAKE) fixlabels
	# @echo Compiling SUP for bibliography
	# @$(LATEX) $(SUP)
	# @echo Generating bibliography
	# @$(BIBTEX) $(SUP)
	# @echo Recompiling SUP after generating bibliography
	# @$(LATEX)  $(SUP)
	# @$(MAKE) fixlabels

%.eps.pdf: %.eps
	@echo "	" Converting $< to $(@)
	@epstopdf --outfile=figs/$(@) $<

clean:
	#@make -C figs clean
	@/bin/rm -f $(MAIN).ps $(MAIN).pdf *.aux *.dvi *.log *.bbl *.blg figs/*.pdf figures/plot/*.pdf *.toc *.out *.bak


==> dl_am.tex <==
%\subsection{Deep learning in Speech Recognition}
%\label{ref:sec:back:dl_am}
Neural networks with deep architectures have been the dominant acoustic modeling approach for automatic speech recognition (ASR) in recent years. They have yielded state-of-the-art performance as compared to previous technologies based on hidden Markov models (HMMs) and Gaussian mixtures \cite{Hinton_DNNSPM}. In some tasks, Deep Learning (DL) has achieved near human-level ASR performance \cite{saon-interspeech-2017, msr-speech}. It is commonly agreed that the success of DL for ASR relies on the availability of large amount of training data and high-performance computing. Therefore, distributed DL is not only preferred but also necessary in DL ASR to guarantee fast turnaround time for model training. 


==> power_meth.tex <==
%PyTorch 0.5.0 is the underlying DL framework. We use the CUDA 9.2 compiler, the CUDA-aware OpenMPI 3.1.1, and g++ 4.8.5 compiler to build our communication library, which connects with PyTorch via a Python-C interface. 

%We develop and experiment our systems on a production-run cluster \dyce, which has 4 servers in total. Each server is equipped with 14-core Intel Xeon E5-2680 v4 2.40GHz processor, 1TB main memory, and 4 P100 GPUs.

%IBM POWER9 CPUs and NVIDIA Volta GPUs all connected together with NVIDIA’s high-speed NVLink.
%Interconnect Topology: Mellanox EDR 100G InfiniBand, Non-blocking
%The basic building block of Summit is the IBM Power System AC922 node. Each of the approximately 4,600 compute nodes on Summit contains two IBM POWER9 processors and six NVIDIA Volta V100 accelerators and provides a theoretical double-precision capability of approximately 40 TF. Each POWER9 processor is connected via dual NVLINK bricks, each capable of a 25GB/s transfer rate in each direction. Nodes contain 512 GB of DDR4 memory for use by the POWER9 processors and 96 GB of High Bandwidth Memory (HBM2) for use by the accelerators. Additionally, each node has 1.6TB of non-volatile memory that can be used as a burst buffer.

We also present 48-GPU results on an experimental IBM cluster \wsc with a node
architecture similar to the current fastest supercomputer in the world, Summit
\cite{Top500}. This cluster is based on IBM POWER System AC922 nodes with IBM
POWER9 CPUs and NVIDIA Volta V100 GPUs all connected together with NVIDIA’s
high-speed NVLink dual links totaling 50GB/s bandwidth in each direction.
Nodes are connected with Mellanox EDR 100G Infiniband interconnect technology.
For the POWER9 cluster, different from the other clusters we use PyTorch v1.0.0
and IBM IBM Spectrum MPI along with XL compiler suite v16.1.1 based on
availability.


==> power_results.tex <==
\subsection{Speedup}
\begin{figure}[t]%[!htpb]
  \centering
    {\includegraphics[width=1.0\columnwidth]{./figures/speedup_wsc_batch160}
      \caption{Speedup up to 96 gpus from POWER9 cluster}
    \label{fig:SpeedupWSC}
    }
\end{figure}


==> xiaodong.tex <==
The mathematical model of ADPSGD is given in Eq.\ref{eqn:adpsgd}
\begin{align}
    \Theta_{k+1} = \Theta_{k}T_{k} - \alpha_{k}\partial G(\Theta_{k},\bm{\Xi}_{k})  \label{eqn:adpsgd}
\end{align}
where $n$ is the total number of learners; the columns of $\Theta_{k} = [\theta^{1}_{k}, \cdots, \theta^{n}_{k}]$ are weights of each learner; the columns of $\Xi_{k} = [\xi^{1}_{k}, \cdots, \xi^{n}_{k}]$ are random variables associated with batch samples; the columns of $\partial G(\Theta_{k},\bm{\Xi}_{k})  = [\nabla F(\theta^{1}_{k},\xi^{1}_{k}), \cdots, \nabla F(\theta^{n}_{k},\xi^{n}_{k})]$ are gradients of each learner and $T_{k}$ is a symmetric stochastic matrix (therefore doubly stochastic) with two $0.5$'s at neighboring positions for each row and column.

ADPSGD is carried out with local gradient computation and update on each learner (second term on the RHS of Eq.\ref{eqn:adpsgd}) and global model averaging (first term of the RHS of Eq.\ref{eqn:adpsgd}) across the ring. The locally updated information is transferred to other learners in the ring by performing model averaging through neighboring learners. If we halt the local updates and only conduct the model averaging through the doubly stochastic matrix $T_{k}$, the system will converge to the equilibrium where all learners share the identical weights which is $\frac{1}{n}\sum_{i=1}^{n}\theta^{i}_{k}$. After the convergence, each learner pulls the weights, compute gradients, update the model and conducts another round of model averaging to convergence. This amounts to synchronous SGD. Therefore, ADPSGD has synchronous SGD as its special case. However, in ADPSGD, local updates and model averaging runs simultaneously. It can be interpreted that the local updates are carried out on $\frac{1}{n}\sum_{i=1}^{n}\theta^{i}_{k}$ perturbed by a noise term. This might help optimization use larger batch size that is not possible for synchronous SGD.    
